Unit Commitment With Gas Network Awareness

Recent changes in the fuel mix for electricity generation and, in particular, the increase in Gas-Fueled Power Plants (GFPP), have created significant interdependencies between the electrical power and natural gas transmission systems. However, despite their physical and economic couplings, these networks are still operated independently, with asynchronous market mechanisms. This mode of operation may lead to significant economic and reliability risks in congested environments as revealed by the 2014 polar vortex event experienced by the northeastern United States. To mitigate these risks, while preserving the current structure of the markets, this paper explores the idea of introducing gas network awareness into the standard unit commitment model. Under the assumption that the power system operator has some (or full) knowledge of gas demand forecast and the gas network, the paper proposes a tri-level mathematical program where natural gas zonal prices are given by the dual solutions of natural-gas flux conservation constraints and commitment decisions are subject to bid-validity constraints that ensure the economic viability of the committed GFPPs. This tri-level program can be reformulated as a single-level Mixed-Integer Second-Order Cone program which can then be solved using a dedicated Benders decomposition. The approach is validated on a case study for the Northeastern United States [1] that can reproduce the gas and electricity price spikes experienced during the early winter of 2014. The results on the case study demonstrate that gas awareness in unit commitment is instrumental in avoiding the peaks in electricity prices while keeping the gas prices to reasonable levels.

==> Literature.tex <==
\section{Literature review}
Recently, there have been several studies that incorporate the natural gas transmission feasibility into unit commitment models via some decomposition techniques or co-optimizing these coupled systems \citep{liu2009security, li2008interdependency, biskas2016coupled}. However, these studies do not address the economic interdependence between these two systems. 

Only a limited number of studies have discussed how to incorporate the market feedback for the gas network into the unit-commitment model. The highly decentralized natural gas markets presents modeling challenges in capturing the feedback, hence \cite{chen2017clearing} and \cite{wang2018equilibrium} proposed a new framework of a joint gas and electricity market that assume centralized natural gas markets. This proposed work, on the other hand, aims to develop a unit-commitment model that is aware of the natural gas clearing price, which can be readily applicable to the current power system.   

%(not market, but the network constraints) Geidl \& Andersson (2007) and incorporate natural gas network constraints in the optimal power flow problem, while the unit commitment problem with natural gas security constraints is solved by Liu et al. (2009) and Li et al. (2008). 


%Existing economic models of natural gas trade have generally relied on one of two approaches to obtain tractable equilibrium solutions to gas market problems. Some existing work has consrtructed large-scale optimization models of trade on natural gas transmission systems. These models are often formulated as mixed complementarity problems [23, 24, 25, 26, 27]. A second approach has been to develop dynamic general or partial equilibrium trade models of natural gas markets. These models have primarily (but not always) been used to examine global trade in natural gas [28, 29, 30].

%The aforementioned contributions utilize a steady-state approach to model the natural gas system which may result in suboptimal solutions when considering short-term operations. In contrast to the electricity system, natural gas can be stored in the network and moves with a lower speed than electricity. These characteristics are important as they endow the natural gas system with flexibility that can be exploited to ensure reliability; especially in cases of highly variable withdrawals by the GFPPs. Liu et al. (2011) and Chaudry et al. (2008) model a dynamic natural gas system with linepack (i.e., ability of storing natural gas in the pipelines) by solving a mixed-integer nonlinear and a nonlinear program, respectively. However, these approaches do not guarantee global optimal solutions, involve high computation times and are not suitable to be included in a market mechanism as it is hard to derive prices from them. Additionally, Correa-Posada & Sanchez-Martin (2014) propose a linearization approach based on mixed-integer linear programming to efficiently approximate a dynamic natural gas model that is easier to solve at global optimality. Liu et al. (2009), Li et al. (2008) and Alabdulwahab et al. (2015) consider the natural gas network constraints only to ensure feasibility and do not optimize the operational cost of the natural gas system. Hence, the optimal operation of the integrated energy system is not guaranteed.


